A Multiwavelength Classification and Study of Red Supergiant Candidates in NGC 6946

We have combined resolved stellar photometry from Hubble Space Telescope (\emph{HST}), \emph{Spitzer}, and \emph{Gaia} to identify red supergiant (RSG) candidates in NGC~6946, based on their colors, proper motions, visual morphologies, and spectral energy distributions. We start with a large sample of 17,865 RSG candidates based solely on \emph{HST} near-infrared photometry. We then chose a small sample of 385 of these candidates with Spitzer matches for more detailed study. Using evolutionary models and isochrones, we isolate a space where RSGs would be found in our photometry catalogs. We then visually inspect each candidate and compare to Gaia catalogs to identify and remove foreground stars. As a result, we classify 95 potential RSGs, with 40 of these being in our highest-quality sample. We fit the photometry of the populations of stars in the regions surrounding the RSGs to infer their ages. Placing our best candidate RSG stars into three age bins between 1 and 30 Myr, we find 27.5\% of the candidates falling between 1-10 Myr, 37.5\% between 10-20 Myr, and 35\% 20-30 Myr. A comparison of our results to the models of massive star evolution shows some agreement between model luminosities and the luminosities of our candidates for each age. Three of our candidates appear significantly more consistent with binary models than single-star evolution models.

==> Tables/MATCH_results.tex <==
\begin{center}
\begin{longtable}{cccccc}
\caption{Full list of results from MATCH. Column 5 is a flag indicating the status of a candidate. A means the candidate has shown only signs of being a quality candidate. B indicates the candidate is in a potential binary system, C means the star is a potential low mass contaminant (AGB star), D means the candidate location was analyzed with the F435W and F606W filter combination, F means the star is a potential foreground star, M indicates the candidates that were our most likely mismatches, and IN means the the location had insufficient coverage in the surrounding area to get an age estimate from MATCH. A flag of 1 means the candidate belongs to the primary sample comprised of only single matches between HST and Spitzer sources while 2 means the candidate belongs to the secondary sample of candidates that had multiple matches between HST and Spitzer sources. \label{tab:MATCH_results}} \\ 
\hline
\hline
Identifier & $dA_{v}$ & $A_{v}$ & Age (Myr) & Flags \\
\hline
\endfirsthead
\hline
\multicolumn{5}{c}{Continuation of Table \ref{tab:MATCH_results}}\\
\hline
Identifier & $dA_{v}$ & $A_{v}$ & Age (Myr) & Flags \\
\hline
\endhead
\hline
\endfoot
\hline
\endlastfoot
RSG 2669 &  0.2 &  1.15 &   16 &       M,2 \\
 RSG 2055 &    2 &  2.35 &    4 &       F,2 \\
 RSG 6602 &  0.2 &   1.4 &    0 &       C,1 \\
 RSG 1851 &    0 &   1.5 &   11 &       M,2 \\
 RSG 6318 &    0 &  1.65 &   18 &       A,1 \\
 RSG 1278 &    0 &   1.2 &   26 &       F,1 \\
 RSG 3066 &  0.2 &   1.6 &   16 &       M,2 \\
 RSG 1356 &  0.4 &   1.5 &   13 &       A,2 \\
  RSG 650 &  0.8 &   1.6 &    5 &       M,2 \\
 RSG 2214 &  0.2 &  1.35 &   27 &     A,D,1 \\
 RSG 6822 &    0 &   1.5 &   12 &     A,D,1 \\
  RSG 356 &  0.4 &   0.9 &   13 &       M,1 \\
 RSG 1198 &  0.2 &  1.05 &   13 &       M,2 \\
 RSG 4741 &  N/A &   N/A &  N/A &  D,M,IN,1 \\
 RSG 4906 &    0 &  1.05 &   11 &     A,D,1 \\
   RSG 56 &    1 &     1 &    9 &       F,2 \\
  RSG 347 &  1.6 &  1.35 &   29 &     D,F,1 \\
 RSG 1764 &    0 &  1.05 &    4 &       M,1 \\
 RSG 1785 &  0.4 &  1.75 &    0 &     C,D,1 \\
 RSG 4325 &    0 &  1.55 &   19 &       M,1 \\
 RSG 6222 &  0.2 &  1.55 &    0 &       C,1 \\
 RSG 4825 &  N/A &   N/A &  N/A &    D,IN,1 \\
 RSG 3223 &  1.2 &  1.25 &   29 &     D,M,1 \\
 RSG 5027 &    0 &  1.25 &    0 &       C,1 \\
 RSG 2398 &    0 &  1.85 &   16 &       F,1 \\
 RSG 5026 &    0 &  1.15 &   29 &     A,D,1 \\
 RSG 5542 &    0 &   1.5 &   16 &       A,2 \\
 RSG 3282 &    0 &  1.85 &   21 &       A,1 \\
 RSG 1590 &    0 &   2.1 &    7 &       F,2 \\
 RSG 4203 &    0 &   1.4 &   23 &       M,2 \\
 RSG 3991 &  1.2 &   1.5 &    5 &       A,1 \\
 RSG 3984 &  N/A &   N/A &  N/A &    D,IN,1 \\
 RSG 2813 &    0 &  1.15 &   26 &       A,1 \\
 RSG 1900 &  0.4 &   1.5 &    4 &     D,M,2 \\
 RSG 5871 &    0 &   1.5 &    9 &     D,M,2 \\
 RSG 2666 &    0 &   1.2 &   15 &       A,2 \\
  RSG 422 &  0.8 &   1.6 &    0 &     C,F,1 \\
 RSG 2788 &  1.2 &  2.15 &    6 &       F,1 \\
 RSG 2965 &  0.4 &   1.9 &   27 &     D,F,1 \\
 RSG 1839 &    0 &   1.4 &   15 &       M,1 \\
 RSG 6480 &  0.4 &   1.1 &   11 &       M,2 \\
 RSG 3105 &    0 &   1.5 &   17 &     A,D,2 \\
 RSG 4781 &    0 &  1.35 &    5 &       A,1 \\
 RSG 5914 &  N/A &   N/A &  N/A &  D,M,IN,1 \\
 RSG 2768 &  0.4 &  2.05 &   23 &       A,1 \\
 RSG 2841 &    0 &     1 &    4 &       A,1 \\
 RSG 4393 &  1.2 &  1.05 &   13 &     A,D,2 \\
 RSG 1282 &    0 &   1.3 &   14 &       A,1 \\
  RSG 477 &    0 &     1 &    8 &       F,1 \\
 RSG 2132 &    0 &  2.15 &   15 &     D,M,2 \\
 RSG 1966 &    0 &   1.5 &    5 &       A,1 \\
 RSG 1321 &    0 &   1.6 &   15 &       A,1 \\
 RSG 3485 &    0 &   1.3 &    9 &     A,D,1 \\
 RSG 2171 &  0.2 &   1.8 &   16 &       A,1 \\
 RSG 1132 &    0 &   1.6 &   23 &       M,2 \\
 RSG 3129 &    0 &   1.5 &   13 &       M,2 \\
 RSG 2464 &    0 &   1.7 &    5 &       M,2 \\
 RSG 3160 &  0.2 &   0.9 &   16 &       A,1 \\
 RSG 2556 &    0 &  1.85 &   13 &       M,2 \\
 RSG 4972 &    0 &   1.4 &   16 &       A,1 \\
  RSG 611 &  1.6 &   1.6 &    4 &     D,F,1 \\
 RSG 3759 &  1.2 &   1.8 &   27 &       A,2 \\
 RSG 3532 &    0 &  1.55 &   29 &     A,D,1 \\
 RSG 3059 &  2.2 &  1.75 &   15 &     A,D,1 \\
 RSG 3561 &    0 &  1.15 &   16 &       A,1 \\
 RSG 4502 &    0 &  1.35 &   29 &       A,1 \\
  RSG 997 &  1.2 &   1.1 &   17 &       F,2 \\
  RSG 814 &  N/A &   N/A &  N/A &    D,IN,1 \\
  RSG 959 &    0 &   1.1 &    7 &       M,1 \\
  RSG 350 &    0 &   1.6 &    5 &       M,1 \\
 RSG 2218 &  0.4 &  1.15 &    4 &       M,2 \\
 RSG 2748 &    0 &     2 &   21 &     A,D,1 \\
  RSG 578 &  0.8 &   0.8 &   15 &       F,1 \\
  RSG 309 &  2.6 &   2.3 &    4 &       F,2 \\
 RSG 1465 &  N/A &   N/A &  N/A &  D,F,IN,2 \\
  RSG 759 &  0.8 &   0.9 &   23 &       M,2 \\
 RSG 4176 &    0 &  1.15 &   16 &       M,2 \\
 RSG 2424 &    0 &  1.15 &   14 &       A,1 \\
   RSG 51 &  N/A &   N/A &  N/A &  D,F,IN,1 \\
 RSG 1622 &    0 &   1.8 &    6 &       M,1 \\
  RSG 798 &  0.2 &  1.15 &    5 &     D,F,1 \\
 RSG 1355 &  0.2 &  0.85 &   10 &     A,D,1 \\
 RSG 1661 &  0.4 &   1.7 &    5 &       A,1 \\
  RSG 928 &    0 &  1.95 &   24 &     A,D,1 \\
  RSG 542 &  N/A &   N/A &  N/A &  D,M,IN,1 \\
 RSG 1592 &    0 &  1.25 &    4 &     A,D,2 \\
 RSG 5460 &    0 &  1.35 &   16 &       A,1 \\
 RSG 2722 &    0 &  1.55 &   21 &       M,1 \\
 RSG 3935 &  1.4 &  1.05 &   24 &     D,M,1 \\
  RSG 383 &  0.4 &  1.35 &   24 &     D,F,1 \\
 RSG 2006 &    0 &   1.3 &   19 &       M,2 \\
  RSG 935 &    0 &  1.45 &   17 &     D,M,1 \\
 RSG 2226 &    0 &  1.25 &    8 &     D,F,1 \\
 RSG 1385 &    0 &  1.65 &    6 &       M,1 \\
 RSG 5007 &    0 &  1.35 &   10 &       M,1 \\
 RSG 1539 &  0.2 &   1.6 &    5 &       A,1 \\
 RSG 2680 &  0.2 &   0.8 &    4 &       A,2 \\
 RSG 3158 &    0 &  0.95 &    0 &       C,1 \\
  RSG 527 &  0.8 &   1.4 &    4 &     D,M,1 \\
 RSG 2141 &    0 &  1.45 &    5 &     D,M,2 \\
  RSG 734 &    0 &  1.45 &    5 &     D,F,1 \\
 RSG 3954 &    0 &     1 &   10 &       A,1 \\
 RSG 4092 &  0.4 &   1.6 &   13 &       F,2 \\
 RSG 1919 &  1.6 &  1.05 &    5 &     D,M,2 \\
 RSG 3091 &    0 &  1.65 &    6 &       A,1 \\
 RSG 1489 &    0 &   1.4 &    0 &       C,1 \\
 RSG 4665 &  N/A &   N/A &  N/A &    D,IN,1 \\
 RSG 4480 &  0.2 &   1.5 &   26 &       A,1 \\
 RSG 2276 &    0 &  1.55 &   21 &       A,2 \\
 RSG 4966 &  N/A &   N/A &  N/A &    D,IN,1 \\
 RSG 5120 &  1.4 &  1.15 &   14 &       A,2 \\
 RSG 4949 &    0 &   1.6 &    9 &       A,1 \\
 RSG 5381 &    1 &   2.1 &    6 &     D,M,1 \\
  RSG 694 &  0.2 &   1.5 &   13 &     D,M,2 \\
  RSG 677 &  1.8 &   2.6 &   24 &     D,F,1 \\
 RSG 1534 &  1.6 &  1.45 &    4 &       A,1 \\
 RSG 4118 &  0.2 &   2.1 &   29 &       A,1 \\
  RSG 637 &  0.2 &   0.9 &    4 &     D,F,1 \\
 RSG 4489 &  1.2 &   1.8 &    0 &       C,1 \\
 RSG 3640 &  N/A &   N/A &  N/A &    D,IN,1 \\
  RSG 692 &    0 &  1.05 &    6 &     D,F,2 \\
  RSG 447 &    0 &   1.3 &    4 &     D,F,1 \\
 RSG 3441 &  N/A &   N/A &  N/A &    D,IN,1 \\
 RSG 1930 &    0 &   1.3 &    0 &     C,M,1 \\
 RSG 3264 &    0 &  1.35 &   11 &     D,F,1 \\
 RSG 4623 &    0 &  1.45 &   29 &     A,D,1 \\
 RSG 1713 &  0.2 &   1.8 &   26 &       F,1 \\
 RSG 3199 &    0 &   1.5 &   14 &     D,M,2 \\
 RSG 767 &  0.4 &  1.65 &    9 &     A,D,1 \\
 RSG 1480 &    0 &   1.3 &    4 &     D,F,1 \\
 RSG 1189 &    0 &   1.6 &    4 &     D,F,1 \\
 RSG 4881 &    0 &  1.55 &   27 &     A,D,1 \\
 RSG 1744 &  0.2 &   1.1 &   19 &       F,2 \\
 RSG 3335 &    0 &   1.1 &   13 &     A,D,1 \\
 RSG 3163 &    0 &  1.15 &   21 &     D,F,2 \\
 RSG 3336 &  1.2 &   0.8 &   23 &       A,1 \\
 RSG 3113 &    0 &  1.05 &   16 &       A,2 \\
\end{longtable}
\end{center}

==> Tables/Observations.tex <==
\startlongtable 
\begin{longrotatetable}
\begin{deluxetable}{cccccccc} 
\tablewidth{0pt} 
\tablecolumns{8} 
\tablecaption{NGC 6946 Observations} 
\tablehead{
\colhead{Image} & \colhead{PID} & \colhead{Date} & \colhead{RA (J2000)} & \colhead{Dec (J2000)} & \colhead{V3 Axis (deg)} & \colhead{Exp Time (sec)} & \colhead{Filter} }
\startdata
icyq02g6q & 14156 & 2016-02-09 & 308.74498 & 60.10888 & 166.93769 & 228 & WFC3 F110W \\
icyq02g8q & 14156 & 2016-02-09 & 308.74427 & 60.11086 & 166.93690 & 228 & WFC3 F110W \\
icyq02h1q & 14156 & 2016-02-09 & 308.68559 & 60.12741 & 166.88609 & 228 & WFC3 F110W \\
icyqa2h3q & 14156 & 2016-02-09 & 308.68441 & 60.12877 & 166.81579 & 228 & WFC3 F110W \\
icyqa2hdq & 14156 & 2016-02-09 & 308.62572 & 60.14583 & 166.76489 & 228 & WFC3 F110W \\
icyqa2hfq & 14156 & 2016-02-09 & 308.62489 & 60.14722 & 166.76421 & 228 & WFC3 F110W \\
icyqb2hoq & 14156 & 2016-02-09 & 308.65851 & 60.17230 & 166.74741 & 228 & WFC3 F110W \\
icyqb2hqq & 14156 & 2016-02-09 & 308.65768 & 60.17369 & 166.74659 & 228 & WFC3 F110W \\
icyqc2hzq & 14156 & 2016-02-09 & 308.71798 & 60.15385 & 166.77150 & 228 & WFC3 F110W \\
icyqc2i1q & 14156 & 2016-02-09 & 308.71715 & 60.15525 & 166.77071 & 228 & WFC3 F110W \\
icyqd2iaq & 14156 & 2016-02-09 & 308.77755 & 60.13539 & 166.78489 & 228 & WFC3 F110W \\
icyqd2icq & 14156 & 2016-02-09 & 308.77672 & 60.13678 & 166.78410 & 228 & WFC3 F110W \\
icyqd2ilq & 14156 & 2016-02-09 & 308.80985 & 60.16186 & 166.81289 & 228 & WFC3 F110W \\
icyqd2inq & 14156 & 2016-02-09 & 308.80902 & 60.16325 & 166.81210 & 228 & WFC3 F110W \\
icyqe2iwq & 14156 & 2016-02-09 & 308.75020 & 60.18035 & 166.68691 & 228 & WFC3 F110W \\
icyqe2iyq & 14156 & 2016-02-09 & 308.74936 & 60.18175 & 166.68609 & 228 & WFC3 F110W \\
icyqe2j7q & 14156 & 2016-02-09 & 308.69052 & 60.19874 & 166.63510 & 228 & WFC3 F110W \\
icyqf2j8q & 14156 & 2016-02-09 & 308.68956 & 60.20002 & 166.55819 & 228 & WFC3 F110W \\
id6o01lzq & 14638 & 2016-10-23 & 308.62762 & 60.13978 & 256.69132 & 99 & WFC3 F160W \\
id6o01m2q & 14638 & 2016-10-23 & 308.62796 & 60.13983 & 256.69159 & 99 & WFC3 F160W \\
id6o01m5q & 14638 & 2016-10-23 & 308.63039 & 60.14019 & 256.69369 & 99 & WFC3 F160W \\
id6o01m8q & 14638 & 2016-10-23 & 308.63073 & 60.14025 & 256.69400 & 99 & WFC3 F160W \\
id6o02mdq & 14638 & 2016-10-23 & 308.66598 & 60.17140 & 256.72449 & 99 & WFC3 F160W \\
id6o02mgq & 14638 & 2016-10-23 & 308.66633 & 60.17145 & 256.72479 & 99 & WFC3 F160W \\
id6o02mjq & 14638 & 2016-10-23 & 308.66875 & 60.17182 & 256.72689 & 99 & WFC3 F160W \\
id6o02mmq & 14638 & 2016-10-23 & 308.66909 & 60.17187 & 256.72720 & 99 & WFC3 F160W \\
id6o03b1q & 14638 & 2016-10-24 & 308.70423 & 60.20295 & 256.75781 & 99 & WFC3 F160W \\
id6o03b4q & 14638 & 2016-10-24 & 308.70457 & 60.20300 & 256.75809 & 99 & WFC3 F160W \\
id6o03b7q & 14638 & 2016-10-24 & 308.70701 & 60.20336 & 256.76019 & 99 & WFC3 F160W \\
id6o03bdq & 14638 & 2016-10-24 & 308.70735 & 60.20342 & 256.76049 & 99 & WFC3 F160W \\
id6o04gmq & 14638 & 2016-10-25 & 308.68339 & 60.12258 & 256.73969 & 99 & WFC3 F160W \\
id6o04gpq & 14638 & 2016-10-25 & 308.68373 & 60.12263 & 256.73999 & 99 & WFC3 F160W \\
id6o04gsq & 14638 & 2016-10-25 & 308.68616 & 60.12299 & 256.74209 & 99 & WFC3 F160W \\
id6o04gvq & 14638 & 2016-10-25 & 308.68649 & 60.12305 & 256.74240 & 99 & WFC3 F160W \\
id6o05j4q & 14638 & 2016-10-26 & 308.72163 & 60.15416 & 256.77289 & 99 & WFC3 F160W \\
id6o05jbq & 14638 & 2016-10-26 & 308.72196 & 60.15421 & 256.77329 & 99 & WFC3 F160W \\
id6o05jfq & 14638 & 2016-10-26 & 308.72439 & 60.15457 & 256.77539 & 99 & WFC3 F160W \\
id6o05k5q & 14638 & 2016-10-26 & 308.72473 & 60.15462 & 256.77569 & 99 & WFC3 F160W \\
id6o06kcq & 14638 & 2016-10-26 & 308.76007 & 60.18579 & 256.80631 & 99 & WFC3 F160W \\
id6o06kjq & 14638 & 2016-10-26 & 308.76041 & 60.18585 & 256.80648 & 99 & WFC3 F160W \\
id6o06knq & 14638 & 2016-10-26 & 308.76284 & 60.18621 & 256.80869 & 99 & WFC3 F160W \\
id6o06kqq & 14638 & 2016-10-26 & 308.76318 & 60.18626 & 256.80899 & 99 & WFC3 F160W \\
id6o07nhq & 14638 & 2016-10-27 & 308.73893 & 60.10533 & 256.78809 & 99 & WFC3 F160W \\
id6o07nkq & 14638 & 2016-10-27 & 308.73927 & 60.10538 & 256.78830 & 99 & WFC3 F160W \\
id6o07nnq & 14638 & 2016-10-27 & 308.74169 & 60.10574 & 256.79041 & 99 & WFC3 F160W \\
id6o07nqq & 14638 & 2016-10-27 & 308.74204 & 60.10579 & 256.79071 & 99 & WFC3 F160W \\ 
id6o08ntq & 14638 & 2016-10-27 & 308.77688 & 60.13697 & 256.82128 & 99 & WFC3 F160W \\
id6o08nwq & 14638 & 2016-10-27 & 308.77722 & 60.13702 & 256.82159 & 99 & WFC3 F160W \\
id6o08nzq & 14638 & 2016-10-27 & 308.77965 & 60.13738 & 256.82370 & 99 & WFC3 F160W \\
id6o08o2q & 14638 & 2016-10-27 & 308.77999 & 60.13743 & 256.82401 & 99 & WFC3 F160W \\
id6o09o5q & 14638 & 2016-10-27 & 308.81592 & 60.16851 & 256.85471 & 99 & WFC3 F160W \\
id6o09o8q & 14638 & 2016-10-27 & 308.81626 & 60.16856 & 256.85501 & 99 & WFC3 F160W \\
id6o09obq & 14638 & 2016-10-27 & 308.81869 & 60.16893 & 256.85709 & 99 & WFC3 F160W \\
id6o09oeq & 14638 & 2016-10-27 & 308.81903 & 60.16898 & 256.85739 & 99 & WFC3 F160W \\
id9g03l6q & 15216 & 2016-10-26 & 308.85714 & 60.11530 & 269.00180 & 680 & ACS F606W \\ 
id9g03l9q & 15216 & 2016-10-26 & 308.85714 & 60.11530 & 269.00180 & 720 & ACS F606W \\ 
id9g03ldq & 15216 & 2016-10-26 & 308.85714 & 60.11530 & 269.00180 & 720 & ACS F606W \\ 
id9g03lhq & 15216 & 2016-10-26 & 308.85714 & 60.11530 & 269.00171 & 680 & ACS F606W \\ 
idk409djq & 15216 & 2018-12-10 & 308.82705 & 60.18438 & 209.16740 & 900 & ACS F606W \\ 
idk409dmq & 15216 & 2018-12-10 & 308.82641 & 60.18360 & 209.16690 & 910 & ACS F606W \\ 
idk409dsq & 15216 & 2018-12-10 & 308.82578 & 60.18282 & 209.16631 & 900 & ACS F606W \\ 
idk409e0q & 15216 & 2018-12-10 & 308.82705 & 60.18438 & 209.16740 & 950 & ACS F814W \\ 
idk409e5q & 15216 & 2018-12-10 & 308.82641 & 60.18360 & 209.16690 & 950 & ACS F814W \\ 
idk409eaq & 15216 & 2018-12-10 & 308.82578 & 60.18282 & 209.16631 & 950 & ACS F814W \\ 
idk409eeq & 15216 & 2018-12-10 & 308.82705 & 60.18438 & 209.16740 & 950 & ACS F606W \\ 
idk409eiq & 15216 & 2018-12-10 & 308.82641 & 60.18360 & 209.16690 & 950 & ACS F606W \\ 
idk409emq & 15216 & 2018-12-10 & 308.82578 & 60.18282 & 209.16631 & 950 & ACS F606W \\ 
idk409eqq & 15216 & 2018-12-10 & 308.82705 & 60.18438 & 209.16740 & 950 & ACS F814W \\ 
idk409euq & 15216 & 2018-12-10 & 308.82641 & 60.18360 & 209.16690 & 950 & ACS F814W \\ 
idk409eyq & 15216 & 2018-12-10 & 308.82578 & 60.18282 & 209.16631 & 950 & ACS F814W \\ 
jbky01gjq & 12331 & 2010-08-24 & 308.80594 & 60.19238 & 346.99951 & 521 & ACS F814W \\ 
jbky01gmq & 12331 & 2010-08-24 & 308.80604 & 60.19222 & 346.99960 & 603 & ACS F814W \\ 
jbky01gqq & 12331 & 2010-08-24 & 308.80613 & 60.19206 & 346.99970 & 603 & ACS F814W \\ 
jbky01gtq & 12331 & 2010-08-24 & 308.80575 & 60.19233 & 346.99939 & 703 & ACS F814W \\ 
jbok05oaq & 12450 & 2012-08-30 & 308.74999 & 60.20574 & 328.98950 & 521 & ACS F814W \\ 
jbok05oeq & 12450 & 2012-08-30 & 308.75025 & 60.20565 & 328.98969 & 600 & ACS F814W \\ 
jbok05p2q & 12450 & 2012-08-30 & 308.75010 & 60.20558 & 328.98959 & 600 & ACS F814W \\ 
jbok05p5q & 12450 & 2012-08-30 & 308.75014 & 60.20581 & 328.98969 & 703 & ACS F814W \\ 
jd9g01s5q & 14786 & 2016-10-28 & 308.80193 & 60.17124 & 277.09921 & 600 & ACS F606W \\ 
jd9g01s8q & 14786 & 2016-10-28 & 308.80193 & 60.17124 & 277.09921 & 690 & ACS F606W \\ 
jd9g01scq & 14786 & 2016-10-28 & 308.80193 & 60.17124 & 277.09921 & 690 & ACS F606W \\ 
jd9g01sgq & 14786 & 2016-10-28 & 308.80193 & 60.17124 & 277.09921 & 590 & ACS F606W \\ 
jd9g01szq & 14786 & 2016-10-28 & 308.80193 & 60.17124 & 277.09921 & 528 & ACS F606W \\ 
jd9g01t2q & 14786 & 2016-10-28 & 308.80193 & 60.17124 & 277.09921 & 690 & ACS F606W \\ 
jd9g01t6q & 14786 & 2016-10-28 & 308.80193 & 60.17124 & 277.09921 & 690 & ACS F606W \\ 
jd9g02r4q & 14786 & 2016-11-02 & 308.74016 & 60.11852 & 277.09891 & 600 & ACS F606W \\ 
jd9g02r7q & 14786 & 2016-11-02 & 308.74016 & 60.11852 & 277.09891 & 690 & ACS F606W \\ 
jd9g02rbq & 14786 & 2016-11-02 & 308.74016 & 60.11852 & 277.09900 & 690 & ACS F606W \\ 
jd9g02rfq & 14786 & 2016-11-02 & 308.74016 & 60.11852 & 277.09900 & 590 & ACS F606W \\ 
jd9g02s6q & 14786 & 2016-11-03 & 308.74016 & 60.11852 & 277.09891 & 538 & ACS F606W \\ 
jd9g02s9q & 14786 & 2016-11-03 & 308.74016 & 60.11852 & 277.09891 & 690 & ACS F606W \\ 
jd9g02sdq & 14786 & 2016-11-03 & 308.74016 & 60.11852 & 277.09900 & 690 & ACS F606W \\ 
jd9g03ktq & 14786 & 2016-10-26 & 308.72317 & 60.18445 & 269.00180 & 530 & ACS F606W \\ 
jd9g03kvq & 14786 & 2016-10-26 & 308.72322 & 60.18448 & 269.00180 & 690 & ACS F606W \\ 
jd9g03kzq & 14786 & 2016-10-26 & 308.72317 & 60.18450 & 269.00180 & 690 & ACS F606W \\ 
jd9g03l3q & 14786 & 2016-10-26 & 308.72312 & 60.18448 & 269.00171 & 520 & ACS F606W \\ 
jd9g03l7q & 14786 & 2016-10-26 & 308.72317 & 60.18445 & 269.00180 & 600 & ACS F814W \\ 
jd9g03laq & 14786 & 2016-10-26 & 308.72322 & 60.18448 & 269.00180 & 690 & ACS F814W \\ 
jd9g03leq & 14786 & 2016-10-26 & 308.72317 & 60.18450 & 269.00180 & 690 & ACS F814W \\ 
jd9g03liq & 14786 & 2016-10-26 & 308.72312 & 60.18448 & 269.00171 & 590 & ACS F814W \\ 
jdk401d3q & 15216 & 2019-01-27 & 308.51700 & 60.11816 & 177.00430 & 816 & ACS F606W \\ 
jdk401d5q & 15216 & 2019-01-27 & 308.51755 & 60.11851 & 177.00481 & 910 & ACS F606W \\ 
jdk401d9q & 15216 & 2019-01-27 & 308.51811 & 60.11885 & 177.00529 & 810 & ACS F606W \\ 
jdk401ddq & 15216 & 2019-01-27 & 308.51700 & 60.11816 & 177.00430 & 900 & ACS F814W \\ 
jdk401dhq & 15216 & 2019-01-27 & 308.51755 & 60.11851 & 177.00481 & 930 & ACS F814W \\ 
jdk401dlq & 15216 & 2019-01-27 & 308.51759 & 60.11848 & 177.00481 & 900 & ACS F814W \\ 
jdk401dpq & 15216 & 2019-01-27 & 308.51704 & 60.11813 & 177.00430 & 987 & ACS F814W \\ 
jdk402vyq & 15216 & 2019-01-25 & 308.60728 & 60.13214 & 177.00430 & 816 & ACS F606W \\ 
jdk402w0q & 15216 & 2019-01-25 & 308.60783 & 60.13249 & 177.00481 & 910 & ACS F606W \\ 
jdk402w4q & 15216 & 2019-01-25 & 308.60839 & 60.13284 & 177.00529 & 810 & ACS F606W \\ 
jdk402w8q & 15216 & 2019-01-25 & 308.60728 & 60.13214 & 177.00430 & 900 & ACS F814W \\ 
jdk402wcq & 15216 & 2019-01-25 & 308.60783 & 60.13249 & 177.00481 & 930 & ACS F814W \\ 
jdk402wgq & 15216 & 2019-01-25 & 308.60788 & 60.13247 & 177.00481 & 900 & ACS F814W \\ 
jdk402wkq & 15216 & 2019-01-25 & 308.60732 & 60.13212 & 177.00430 & 987 & ACS F814W \\ 
jdk404ykq & 15216 & 2019-01-26 & 308.58184 & 60.08963 & 177.00430 & 816 & ACS F606W \\ 
jdk404ymq & 15216 & 2019-01-26 & 308.58239 & 60.08998 & 177.00481 & 910 & ACS F606W \\ 
jdk404yqq & 15216 & 2019-01-26 & 308.58295 & 60.09033 & 177.00529 & 810 & ACS F606W \\ 
jdk404yuq & 15216 & 2019-01-26 & 308.58184 & 60.08963 & 177.00430 & 900 & ACS F814W \\ 
jdk404yyq & 15216 & 2019-01-26 & 308.58239 & 60.08998 & 177.00481 & 930 & ACS F814W \\ 
jdk404z2q & 15216 & 2019-01-26 & 308.58243 & 60.08995 & 177.00481 & 900 & ACS F814W \\ 
jdk404z6q & 15216 & 2019-01-26 & 308.58188 & 60.08961 & 177.00430 & 987 & ACS F814W \\ 
jdk406afq & 15216 & 2019-01-26 & 308.67355 & 60.10451 & 177.00430 & 816 & ACS F606W \\ 
jdk406ahq & 15216 & 2019-01-26 & 308.67411 & 60.10486 & 177.00481 & 910 & ACS F606W \\ 
jdk406alq & 15216 & 2019-01-26 & 308.67466 & 60.10521 & 177.00529 & 810 & ACS F606W \\ 
jdk406arq & 15216 & 2019-01-26 & 308.67355 & 60.10451 & 177.00430 & 900 & ACS F814W \\ 
jdk406avq & 15216 & 2019-01-26 & 308.67411 & 60.10486 & 177.00481 & 930 & ACS F814W \\ 
jdk406azq & 15216 & 2019-01-26 & 308.67415 & 60.10484 & 177.00481 & 900 & ACS F814W \\ 
jdk406b3q & 15216 & 2019-01-26 & 308.67359 & 60.10449 & 177.00430 & 987 & ACS F814W \\ 
jdk407beq & 15216 & 2019-01-26 & 308.64010 & 60.06339 & 177.00430 & 816 & ACS F606W \\ 
jdk407bgq & 15216 & 2019-01-26 & 308.64066 & 60.06374 & 177.00481 & 910 & ACS F606W \\ 
jdk407bkq & 15216 & 2019-01-26 & 308.64121 & 60.06409 & 177.00529 & 810 & ACS F606W \\ 
jdk407boq & 15216 & 2019-01-26 & 308.64010 & 60.06339 & 177.00430 & 900 & ACS F814W \\ 
jdk407bsq & 15216 & 2019-01-26 & 308.64066 & 60.06374 & 177.00481 & 930 & ACS F814W \\ 
jdk407bwq & 15216 & 2019-01-26 & 308.64070 & 60.06372 & 177.00481 & 900 & ACS F814W \\ 
jdk407c7q & 15216 & 2019-01-27 & 308.64015 & 60.06337 & 177.00430 & 987 & ACS F814W \\ 
jdk409diq & 15216 & 2018-12-10 & 308.63330 & 60.16084 & 209.16740 & 859 & ACS F606W \\ 
jdk409dlq & 15216 & 2018-12-10 & 308.63330 & 60.16084 & 209.16690 & 859 & ACS F606W \\ 
jdk409drq & 15216 & 2018-12-10 & 308.63330 & 60.16084 & 209.16631 & 859 & ACS F606W \\ 
jdk409edq & 15216 & 2018-12-10 & 308.63330 & 60.16084 & 209.16740 & 900 & ACS F606W \\ 
jdk409ehq & 15216 & 2018-12-10 & 308.63330 & 60.16084 & 209.16690 & 900 & ACS F606W \\ 
jdk409elq & 15216 & 2018-12-10 & 308.63330 & 60.16084 & 209.16631 & 900 & ACS F606W \\ 
\enddata 
\end{deluxetable} 
\end{longrotatetable}

==> Tables/Phot.tex <==

\begin{table}
\begin{center}
\caption{The first column is a unique identifier for the RSG candidate. The next 4 columns are the RA and DEC in the HST and Spitzer catalogs respectively (J200). The remaining columns are magnitudes in the F435, F606, F814, F110, F160, 3.6m, 4.5m, and 5.8m filters. A value of 99 indicates that the star was not recovered in the filter.}
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c}
\hline
RSG Identifier & RA \emph{HST} & DEC \emph{HST} & RA \emph{Spitzer} & DEC \emph{Spitzer} & F435 Mag & F606 Mag & F814 Mag & F110 Mag & F160 Mag & 3.6$\mu$m Mag & 4.5$\mu$m Mag &  5.8$\mu$m Mag \\ 
\hline\hline
      RSG 2669 &   308.6038821 &     60.1520461 &         308.60391 &           60.15193 &   28.208 &   24.646 &   22.614 &   21.474 &   20.427 &    16.94 &    17.05 &    15.55 \\
      RSG 2055 &   308.6066464 &     60.1462848 &         308.60663 &           60.14621 &   23.972 &   23.081 &    22.27 &    21.36 &   20.354 &    16.64 &    16.69 &     15.9 \\
      RSG 6602 &   308.6109976 &     60.1382102 &         308.61094 &           60.13817 &   27.052 &   24.227 &   22.282 &   21.176 &   20.087 &    18.69 &    18.83 &    16.09 \\
      RSG 1851 &   308.6215717 &     60.1405858 &         308.62158 &           60.14064 &   27.865 &   25.017 &    23.35 &   22.131 &   21.211 &    16.53 &    16.56 &    14.15 \\
      RSG 6318 &   308.6232846 &     60.1269144 &         308.62319 &           60.12691 &   27.666 &   25.533 &   23.223 &   21.522 &   20.498 &    18.36 &    18.67 &    15.87 \\
      RSG 1278 &   308.6236309 &     60.1362338 &         308.62365 &           60.13613 &   26.261 &   24.765 &   23.578 &    22.12 &   21.119 &    16.03 &     16.1 &    13.65 \\
      RSG 3066 &   308.6260371 &     60.1392559 &         308.62595 &           60.13932 &   99.999 &   25.754 &    23.37 &   21.662 &   20.616 &    16.72 &    17.22 &    15.33 \\
      RSG 1356 &   308.6265974 &     60.1384984 &         308.62651 &           60.13855 &   25.909 &   25.245 &   22.927 &   20.987 &   19.795 &    16.14 &    16.17 &    14.62 \\
       RSG 650 &   308.6276566 &     60.1396612 &         308.62766 &            60.1396 &    26.25 &   24.122 &   22.405 &   20.822 &   19.756 &    15.31 &    15.33 &    14.95 \\
      RSG 2214 &   308.6276590 &     60.1714820 &         308.62753 &           60.17153 &   27.506 &   25.941 &   99.999 &   22.321 &   21.252 &    16.72 &    16.79 &    13.93 \\
      RSG 6822 &   308.6299857 &     60.1595435 &         308.62993 &           60.15951 &   99.999 &   27.681 &   99.999 &   21.603 &   20.413 &    18.39 &    18.96 &    16.19 \\
       RSG 356 &   308.6301388 &     60.1380795 &         308.63021 &           60.13805 &   26.809 &   24.728 &   22.753 &   21.396 &   20.433 &    14.53 &    14.78 &    12.95 \\
      RSG 1198 &   308.6302907 &     60.1363369 &         308.63021 &           60.13636 &   26.842 &   25.538 &   23.218 &   21.588 &   20.579 &    15.97 &    16.02 &    13.93 \\
      RSG 4741 &   308.6310596 &     60.1627529 &          308.6312 &           60.16278 &   99.999 &   29.775 &   99.999 &   22.299 &   21.201 &    17.85 &    17.95 &    16.01 \\
      RSG 4906 &   308.6323098 &     60.1629045 &         308.63247 &           60.16302 &   26.637 &   24.644 &   99.999 &   21.002 &   19.956 &    18.01 &    18.02 &    14.94 \\
        RSG 56 &   308.6333372 &     60.1374750 &         308.63337 &            60.1375 &   23.735 &   23.141 &   21.833 &   20.203 &   19.035 &    12.66 &    12.94 &    12.35 \\
       RSG 347 &   308.6347831 &     60.1737147 &         308.63462 &           60.17361 &   99.999 &   25.301 &   99.999 &    21.41 &   20.289 &    14.36 &    14.76 &     11.5 \\
      RSG 1764 &   308.6372782 &     60.1342722 &         308.63729 &           60.13433 &   25.069 &    24.26 &   23.132 &   22.058 &   21.127 &    16.37 &    16.51 &    13.49 \\
      RSG 1785 &   308.6394347 &     60.1697384 &         308.63941 &           60.16976 &   30.238 &   26.023 &   99.999 &   22.074 &   20.921 &    16.43 &    16.52 &    14.07 \\
      RSG 4325 &   308.6397297 &     60.1417534 &         308.63958 &           60.14182 &    28.41 &   26.563 &    23.79 &   21.884 &   20.917 &    17.72 &    17.77 &    15.99 \\
      RSG 6222 &   308.6423098 &     60.1252526 &         308.64223 &           60.12535 &   26.323 &   25.354 &   24.142 &   22.272 &   21.173 &    18.42 &    18.62 &    15.74 \\
      RSG 4825 &   308.6475803 &     60.1875352 &         308.64769 &           60.18753 &   99.999 &   99.999 &   99.999 &   21.496 &   20.286 &    17.76 &    17.98 &    15.43 \\
      RSG 3223 &   308.6481818 &     60.1647505 &         308.64838 &           60.16468 &   27.374 &   25.124 &   99.999 &   21.832 &   20.886 &    16.84 &     17.3 &    16.73 \\
      RSG 5027 &   308.6495598 &     60.1496295 &         308.64945 &           60.14959 &   27.461 &   24.879 &   22.121 &   20.256 &   19.253 &    17.87 &    18.07 &    15.32 \\
      RSG 2398 &   308.6497780 &     60.1507247 &         308.64983 &            60.1508 &   27.161 &    25.38 &   23.187 &   21.587 &   20.625 &    16.69 &     16.9 &    14.48 \\
      RSG 5026 &   308.6503162 &     60.1593026 &         308.65039 &           60.15925 &    27.59 &   23.832 &   99.999 &    20.16 &   19.066 &    17.62 &    18.07 &     13.2 \\
      RSG 5542 &   308.6509015 &     60.1479127 &         308.65078 &           60.14791 &   99.999 &   26.307 &    23.14 &   21.202 &   20.211 &    18.11 &    18.29 &    15.43 \\
      RSG 3282 &   308.6520437 &     60.1569410 &         308.65216 &           60.15698 &   26.302 &   25.051 &   23.278 &   21.522 &   20.433 &    17.23 &    17.33 &    15.29 \\
      RSG 1590 &   308.6527846 &     60.1347001 &         308.65278 &           60.13482 &   23.961 &   23.229 &   22.571 &   22.012 &   20.938 &    16.37 &    16.38 &    15.32 \\
      RSG 4203 &   308.6530159 &     60.1548841 &         308.65293 &           60.15484 &   27.149 &   25.168 &   23.767 &   22.081 &   21.013 &     17.4 &    17.73 &    16.07 \\
      RSG 3991 &   308.6559471 &     60.1528615 &           308.656 &           60.15275 &   27.775 &   24.711 &   22.267 &   20.574 &   19.533 &    17.19 &    17.64 &     15.7 \\
      RSG 3984 &   308.6568806 &     60.1878111 &         308.65693 &           60.18783 &   99.999 &   99.999 &   99.999 &   22.364 &   21.272 &    17.51 &    17.63 &    15.25 \\
      RSG 2813 &   308.6584383 &     60.1221435 &         308.65861 &           60.12224 &   27.088 &   24.549 &   22.077 &   20.536 &   19.385 &    16.85 &    17.11 &    15.12 \\
      RSG 1900 &   308.6591681 &     60.1535855 &         308.65904 &           60.15366 &   27.181 &   25.287 &   99.999 &   22.119 &   21.083 &    16.47 &    16.58 &    14.41 \\
      RSG 5871 &   308.6619373 &     60.1434257 &          308.6618 &            60.1434 &   28.013 &    24.83 &   99.999 &   20.933 &   19.994 &    17.94 &    18.44 &    15.99 \\
      RSG 2666 &   308.6640101 &     60.1857048 &         308.66402 &           60.18568 &   99.999 &   25.356 &   22.641 &   20.872 &   19.893 &    16.49 &    17.05 &    16.83 \\
       RSG 422 &   308.6671856 &     60.1723374 &         308.66723 &           60.17225 &   26.765 &   25.488 &   24.157 &   22.125 &   21.221 &    14.74 &    14.91 &    14.78 \\
      RSG 2788 &   308.6708826 &     60.1573541 &         308.67101 &           60.15728 &   24.868 &   23.872 &   22.866 &   22.024 &   20.934 &    16.79 &     17.1 &    14.76 \\
      RSG 2965 &   308.6717680 &     60.1513484 &         308.67181 &           60.15131 &   25.061 &   23.883 &   99.999 &   21.887 &   20.905 &    17.07 &    17.18 &    15.44 \\
      RSG 1839 &   308.6718111 &     60.1207363 &         308.67178 &           60.12082 &   99.999 &   24.455 &   22.923 &   21.627 &   20.569 &     16.5 &    16.55 &    13.77 \\
      RSG 6480 &   308.6723534 &     60.1566359 &         308.67229 &           60.15655 &   26.062 &   24.087 &   22.797 &   22.174 &   21.178 &    18.28 &    18.75 &    15.56 \\
      RSG 3105 &   308.6753226 &     60.1490551 &         308.67535 &           60.14901 &   24.421 &   23.613 &   99.999 &   21.148 &   20.163 &    17.22 &    17.24 &    14.95 \\
      RSG 4781 &   308.6756799 &     60.1587094 &         308.67567 &           60.15857 &   28.159 &   24.813 &   22.307 &   20.871 &   19.697 &    17.69 &    17.96 &    15.97 \\
      RSG 5914 &   308.6792468 &     60.1384301 &         308.67943 &           60.13848 &   99.999 &   99.999 &   99.999 &    21.11 &   20.107 &    18.15 &    18.46 &    14.92 \\
      RSG 2768 &   308.6792704 &     60.1715049 &         308.67941 &           60.17138 &   28.706 &   25.711 &   23.092 &   21.154 &   20.118 &    16.84 &    17.09 &    14.43 \\
      RSG 2841 &   308.6795178 &     60.1611677 &         308.67929 &            60.1611 &   31.902 &   27.684 &   25.127 &    21.74 &   20.554 &    16.91 &    17.12 &    15.74 \\
      RSG 4393 &   308.6798558 &     60.1470421 &         308.67965 &           60.14712 &   24.158 &   23.531 &   99.999 &   22.109 &   21.134 &    17.51 &     17.8 &    15.64 \\
      RSG 1282 &   308.6802961 &     60.1197923 &         308.68005 &           60.11974 &   25.425 &   24.428 &   22.626 &   21.824 &   20.677 &    16.03 &     16.1 &    14.94 \\
       RSG 477 &   308.6825875 &     60.1214280 &         308.68246 &            60.1215 &   27.463 &   25.983 &   23.447 &   21.436 &   20.298 &    14.92 &    15.06 &    11.52 \\
      RSG 2132 &   308.6861404 &     60.1444217 &         308.68629 &           60.14447 &   28.785 &   25.486 &   99.999 &   21.485 &   20.421 &    16.58 &    16.74 &    13.96 \\
      RSG 1966 &   308.6865859 &     60.1665475 &         308.68637 &           60.16652 &   27.806 &   24.172 &   21.202 &   19.635 &   18.546 &    16.42 &    16.63 &    14.92 \\
      RSG 1321 &   308.6870453 &     60.1269218 &         308.68697 &           60.12679 &   25.283 &   24.121 &   22.587 &   21.246 &   20.229 &    16.01 &    16.14 &    15.36 \\
      RSG 3485 &   308.6882685 &     60.1536417 &         308.68848 &           60.15372 &   99.999 &   26.058 &   99.999 &   21.429 &   20.238 &    17.23 &    17.41 &    15.35 \\
      RSG 2171 &   308.6886474 &     60.1201190 &         308.68851 &           60.12024 &   28.046 &   25.315 &   23.417 &   22.025 &   21.029 &    16.67 &    16.76 &    14.38 \\
      RSG 1132 &   308.6887866 &     60.1707863 &         308.68881 &           60.17078 &   27.547 &   25.051 &   23.146 &   21.703 &    20.75 &    15.91 &    15.95 &    13.94 \\
      RSG 3129 &   308.6889695 &     60.1696087 &         308.68898 &           60.16964 &   27.146 &   25.319 &   23.494 &   22.166 &   21.167 &     17.0 &    17.26 &    14.52 \\
      RSG 2464 &   308.6908817 &     60.1721034 &         308.69084 &           60.17201 &   27.254 &   24.944 &   23.076 &   21.766 &    20.83 &    16.83 &    16.94 &    14.52 \\
      RSG 3160 &   308.6914500 &     60.1637695 &         308.69117 &           60.16378 &   27.137 &   24.804 &   22.873 &   21.324 &    20.37 &    16.96 &    17.28 &    15.34 \\
      RSG 2556 &   308.6941018 &     60.1612310 &         308.69413 &           60.16129 &   28.035 &   25.388 &    23.21 &   21.658 &   20.527 &    16.74 &    16.99 &    14.99 \\
      RSG 4972 &   308.6950166 &     60.1816589 &         308.69505 &           60.18155 &   99.999 &   26.197 &   23.106 &    21.12 &   19.841 &    17.86 &    18.05 &    15.89 \\
       RSG 611 &   308.6958282 &     60.1381605 &         308.69564 &           60.13823 &   27.816 &   25.147 &   99.999 &   21.478 &    20.49 &    15.16 &    15.28 &    14.13 \\
      RSG 3759 &   308.6959172 &     60.1632711 &         308.69586 &           60.16317 &   25.748 &   23.971 &    22.79 &   21.318 &   20.375 &    17.38 &    17.53 &     15.2 \\
      RSG 3532 &   308.7041740 &     60.1438506 &         308.70425 &           60.14396 &   99.999 &   26.199 &   99.999 &   22.306 &   21.234 &    17.41 &    17.43 &    15.57 \\
      RSG 3059 &   308.7042629 &     60.1365304 &         308.70434 &           60.13664 &   25.962 &   24.706 &   99.999 &   22.156 &   20.985 &    17.16 &    17.22 &    15.26 \\
      RSG 3561 &   308.7046380 &     60.1266691 &         308.70474 &            60.1266 &   27.373 &   24.617 &   22.363 &   20.693 &   19.715 &    17.41 &    17.45 &    14.89 \\
      RSG 4502 &   308.7046973 &     60.1794261 &         308.70473 &           60.17949 &   99.999 &   24.967 &    22.87 &   21.516 &   20.539 &    17.39 &    17.86 &    13.99 \\
       RSG 997 &   308.7098625 &     60.1605849 &            308.71 &           60.16047 &   99.999 &     21.1 &   19.999 &   18.931 &   17.871 &    15.57 &    15.81 &    12.41 \\
       RSG 814 &   308.7099131 &     60.1511253 &         308.70972 &           60.15117 &   99.999 &   99.999 &   99.999 &   21.937 &   20.848 &    15.51 &    15.58 &    10.28 \\
       RSG 959 &   308.7105205 &     60.1654891 &         308.71051 &           60.16563 &   99.999 &   25.702 &   23.388 &   21.213 &   20.148 &    15.39 &    15.76 &    12.83 \\
       RSG 350 &   308.7116395 &     60.1606455 &         308.71183 &           60.16062 &   99.999 &   25.416 &   23.218 &   20.925 &   19.881 &    14.75 &    14.76 &    11.54 \\
      RSG 2218 &   308.7137045 &     60.1750969 &         308.71386 &           60.17511 &   99.999 &   25.764 &   23.196 &   21.556 &   20.456 &    16.24 &    16.79 &    15.01 \\
      RSG 2748 &   308.7148431 &     60.1426604 &         308.71467 &           60.14256 &   29.049 &   25.229 &   99.999 &   21.221 &   20.137 &    16.92 &    17.08 &    14.68 \\
       RSG 578 &   308.7149317 &     60.1752593 &         308.71495 &            60.1752 &   99.999 &   23.567 &   21.819 &   20.588 &   19.443 &    14.61 &    15.23 &     14.2 \\
       RSG 309 &   308.7151801 &     60.1656252 &         308.71527 &           60.16563 &   99.999 &   24.059 &   22.843 &   21.432 &   20.385 &    14.58 &    14.67 &    12.66 \\
      RSG 1465 &   308.7162324 &     60.1726299 &          308.7161 &            60.1726 &   99.999 &   99.999 &   99.999 &   21.807 &   20.894 &    16.15 &    16.28 &    16.11 \\
       RSG 759 &   308.7171163 &     60.1667056 &         308.71719 &           60.16661 &   99.999 &    25.34 &   22.786 &   20.921 &   19.823 &    15.38 &    15.49 &    13.36 \\
      RSG 4176 &   308.7181386 &     60.1764494 &         308.71833 &           60.17645 &   99.999 &   25.043 &   22.905 &   21.646 &   20.506 &    17.42 &    17.72 &    14.76 \\
      RSG 2424 &   308.7182381 &     60.1818942 &         308.71807 &           60.18178 &   99.999 &   24.688 &   22.484 &   21.089 &   20.064 &    16.85 &    16.91 &    13.16 \\
        RSG 51 &   308.7189007 &     60.1556360 &         308.71914 &           60.15558 &   99.999 &   99.999 &   99.999 &   21.821 &   20.756 &    12.82 &    12.89 &    10.25 \\
      RSG 1622 &   308.7194166 &     60.1689537 &         308.71925 &           60.16887 &   99.999 &   99.999 &     26.0 &   22.153 &   21.099 &     16.2 &    16.41 &    14.43 \\
       RSG 798 &   308.7246967 &     60.1299560 &         308.72493 &            60.1299 &   26.534 &   24.771 &   99.999 &   21.628 &   20.575 &    15.46 &    15.56 &    13.22 \\
      RSG 1355 &   308.7248032 &     60.1454483 &         308.72467 &           60.14546 &   99.999 &   26.128 &   99.999 &    21.65 &   20.517 &    16.03 &    16.17 &     13.4 \\
      RSG 1661 &   308.7249766 &     60.1689042 &         308.72484 &           60.16887 &   99.999 &   25.026 &   22.481 &   20.684 &   19.734 &    16.36 &    16.45 &    14.91 \\
       RSG 928 &   308.7252642 &     60.1314396 &         308.72538 &           60.13153 &   28.433 &   25.808 &   99.999 &   21.922 &   20.958 &    15.71 &    15.73 &    13.68 \\
       RSG 542 &   308.7262243 &     60.1514096 &         308.72605 &           60.15144 &   99.999 &   99.999 &   99.999 &    22.22 &   21.213 &    15.15 &    15.16 &    12.29 \\
      RSG 1592 &   308.7264454 &     60.1417622 &         308.72643 &           60.14176 &   29.029 &   27.242 &   99.999 &   22.103 &   20.992 &    16.33 &    16.39 &    15.03 \\
      RSG 5460 &   308.7300234 &     60.1851437 &         308.73012 &           60.18504 &   99.999 &   24.756 &    23.04 &   21.739 &   20.668 &    18.05 &    18.25 &    16.17 \\
      RSG 2722 &   308.7310216 &     60.1655087 &         308.73091 &           60.16557 &   99.999 &   26.594 &   24.089 &   22.251 &   21.147 &    16.62 &    17.07 &    16.01 \\
      RSG 3935 &   308.7316522 &     60.1319099 &         308.73162 &           60.13177 &   29.319 &   25.443 &   99.999 &   21.926 &   20.859 &     17.0 &    17.61 &    14.88 \\
       RSG 383 &   308.7336002 &     60.1332455 &         308.73344 &           60.13313 &   25.448 &   24.135 &   99.999 &   21.483 &   20.563 &    14.78 &    14.84 &    14.44 \\
      RSG 2006 &   308.7339026 &     60.1797725 &         308.73403 &           60.17981 &   99.999 &   23.771 &   22.589 &   21.179 &   19.959 &    16.41 &    16.66 &    12.34 \\
       RSG 935 &   308.7341607 &     60.1375460 &         308.73399 &           60.13746 &   28.748 &   25.732 &   99.999 &   21.891 &   20.895 &    15.51 &    15.74 &    12.87 \\
      RSG 2226 &   308.7353687 &     60.1331327 &         308.73544 &           60.13325 &   99.999 &   25.542 &   99.999 &    21.04 &   19.956 &     16.5 &     16.8 &    14.79 \\
      RSG 1385 &   308.7383204 &     60.1926686 &         308.73817 &           60.19257 &   99.999 &   25.473 &   23.424 &   21.839 &   20.913 &    16.19 &    16.21 &    16.62 \\
      RSG 5007 &   308.7434242 &     60.1729180 &         308.74323 &           60.17284 &    23.35 &   22.983 &   21.813 &   20.369 &   19.333 &    17.85 &    18.06 &    14.91 \\
      RSG 1539 &   308.7435525 &     60.1575390 &         308.74347 &           60.15743 &   27.937 &   26.026 &   23.444 &   21.045 &   19.813 &    16.34 &    16.35 &    13.71 \\
      RSG 2680 &   308.7445625 &     60.1715485 &         308.74452 &           60.17161 &   25.066 &   24.402 &   22.984 &    21.75 &   20.815 &    16.86 &    17.05 &    15.14 \\
      RSG 3158 &   308.7450457 &     60.1714463 &         308.74494 &           60.17134 &   26.059 &   24.155 &   21.561 &   19.626 &   18.501 &    16.86 &    17.28 &     14.0 \\
       RSG 527 &   308.7461902 &     60.1446720 &         308.74627 &           60.14476 &   24.971 &   24.178 &   99.999 &   21.334 &   20.152 &    14.77 &    15.13 &    14.27 \\
      RSG 2141 &   308.7467600 &     60.1570854 &         308.74681 &           60.15714 &   26.635 &   25.084 &   99.999 &   22.058 &   21.128 &    16.21 &    16.75 &    14.56 \\
       RSG 734 &   308.7468658 &     60.1448435 &         308.74681 &           60.14493 &   27.343 &    25.49 &   99.999 &   22.085 &   21.194 &    14.77 &    15.44 &    14.87 \\
      RSG 3954 &   308.7481281 &     60.1723855 &         308.74805 &           60.17233 &   28.218 &   25.238 &   23.061 &   21.619 &   20.388 &    17.57 &    17.62 &     16.0 \\
      RSG 4092 &   308.7501761 &     60.1720623 &         308.75022 &             60.172 &   23.114 &   22.771 &    22.16 &    21.45 &   20.382 &    17.17 &    17.68 &    16.19 \\
      RSG 1919 &   308.7519619 &     60.1506588 &         308.75185 &           60.15073 &    27.12 &   24.921 &   99.999 &    21.74 &   20.739 &    16.42 &    16.59 &    15.04 \\
      RSG 3091 &   308.7564013 &     60.1780669 &         308.75619 &           60.17812 &    28.22 &   24.158 &   21.742 &   20.038 &   18.951 &    17.15 &    17.24 &    14.86 \\
      RSG 1489 &   308.7584457 &     60.1761417 &         308.75829 &            60.1761 &   29.777 &   27.509 &   23.796 &   21.056 &   19.948 &    16.23 &     16.3 &    13.68 \\
      RSG 4665 &   308.7631733 &     60.0913454 &         308.76322 &           60.09136 &   99.999 &   26.907 &   99.999 &   22.171 &   21.153 &    17.69 &    17.92 &    15.54 \\
      RSG 4480 &   308.7651006 &     60.1874782 &         308.76517 &           60.18761 &   27.264 &   25.363 &   23.723 &   22.251 &   21.164 &    17.55 &    17.85 &    14.49 \\
      RSG 2276 &   308.7659640 &     60.1665363 &         308.76601 &           60.16648 &   25.238 &    24.18 &   23.199 &   21.982 &   20.977 &    16.76 &    16.83 &    13.25 \\
      RSG 4966 &   308.7686403 &     60.1518182 &          308.7689 &           60.15182 &   28.982 &    25.64 &   99.999 &   22.092 &   21.061 &    17.98 &    18.04 &    16.02 \\
      RSG 5120 &   308.7697077 &     60.1669451 &         308.76956 &           60.16702 &   28.322 &   25.254 &   22.892 &   21.199 &   20.128 &    17.43 &    18.11 &    15.17 \\
      RSG 4949 &   308.7704534 &     60.1665409 &         308.77068 &           60.16648 &    27.99 &   25.853 &   23.009 &   20.677 &   19.524 &    17.85 &    18.03 &    15.24 \\
      RSG 5381 &   308.7755052 &     60.1571028 &         308.77571 &           60.15702 &   99.999 &   99.999 &   99.999 &   22.064 &   20.895 &    18.03 &    18.22 &    15.56 \\
       RSG 694 &   308.7797073 &     60.1238093 &         308.77963 &           60.12376 &   27.141 &   26.219 &   99.999 &   21.821 &   20.879 &    15.12 &     15.4 &     12.9 \\
       RSG 677 &   308.7814770 &     60.1618873 &         308.78151 &           60.16189 &   25.608 &   24.119 &   99.999 &   22.041 &   20.928 &    15.35 &    15.38 &    15.11 \\
      RSG 1534 &   308.7827457 &     60.1651055 &         308.78259 &           60.16509 &    27.94 &   25.828 &   23.019 &   20.528 &   19.517 &    16.31 &    16.34 &    13.82 \\
      RSG 4118 &   308.7845235 &     60.1748893 &         308.78441 &            60.1749 &   27.851 &   23.987 &    21.88 &   20.038 &   19.005 &    17.57 &    17.69 &    15.43 \\
       RSG 637 &   308.7862988 &     60.1626665 &         308.78643 &           60.16269 &   28.569 &   25.138 &   99.999 &   21.499 &   20.433 &    15.29 &    15.31 &    14.17 \\
      RSG 4489 &   308.7874604 &     60.1687846 &         308.78755 &           60.16876 &   27.072 &   25.658 &   24.358 &   22.176 &    21.12 &    17.63 &    17.85 &    15.85 \\
      RSG 3640 &   308.7944655 &     60.1255486 &         308.79452 &           60.12562 &   99.999 &   99.999 &   99.999 &   22.273 &   21.161 &    17.32 &    17.48 &    16.41 \\
       RSG 692 &   308.7957321 &     60.1844984 &         308.79548 &           60.18443 &   24.036 &   23.472 &   99.999 &    21.73 &   20.734 &    15.21 &     15.4 &     13.5 \\
       RSG 447 &   308.7981503 &     60.1627333 &         308.79802 &           60.16285 &   25.176 &   22.367 &   99.999 &   20.174 &   19.095 &    14.97 &    14.99 &    15.07 \\
      RSG 3441 &   308.8002017 &     60.1271411 &         308.80011 &           60.12711 &   99.999 &   99.999 &   99.999 &    22.25 &   21.187 &    17.16 &    17.39 &    15.58 \\
      RSG 1930 &   308.8005506 &     60.1722880 &         308.80034 &           60.17237 &   99.999 &   27.324 &   23.256 &   21.243 &   19.955 &    16.56 &     16.6 &    13.82 \\
      RSG 3264 &   308.8040573 &     60.1606029 &         308.80414 &           60.16061 &   28.892 &   27.165 &   99.999 &   21.797 &   20.819 &    17.21 &    17.32 &    15.86 \\
      RSG 4623 &   308.8084725 &     60.1588447 &         308.80851 &           60.15875 &   28.406 &    25.34 &   99.999 &   22.167 &   21.176 &    17.87 &     17.9 &    16.83 \\
      RSG 1713 &   308.8143668 &     60.1758927 &         308.81416 &           60.17587 &   99.999 &    28.45 &   24.278 &   21.798 &   20.624 &    16.39 &    16.48 &    15.95 \\
      RSG 3199 &   308.8175366 &     60.1802107 &         308.81743 &           60.18026 &   26.546 &   24.884 &   99.999 &   21.924 &   20.837 &    17.27 &    17.29 &    14.78 \\
       RSG 767 &   308.8202537 &     60.1681029 &         308.82012 &           60.16804 &   29.274 &   25.037 &   99.999 &   20.566 &   19.524 &    15.45 &     15.5 &    12.84 \\
      RSG 1480 &   308.8218138 &     60.1538793 &         308.82185 &           60.15397 &   27.668 &   25.427 &   99.999 &   22.281 &   21.214 &    16.21 &    16.29 &    14.55 \\
      RSG 1189 &   308.8253631 &     60.1575448 &         308.82511 &           60.15761 &   27.704 &   25.187 &   99.999 &   21.994 &   20.963 &    15.87 &    16.01 &     16.2 \\
      RSG 4881 &   308.8284572 &     60.1620005 &         308.82835 &           60.16208 &    31.63 &   25.987 &   99.999 &   22.042 &   20.927 &    17.83 &    18.01 &    14.38 \\
      RSG 1744 &   308.8303605 &     60.1710837 &         308.83033 &           60.17111 &    24.53 &   24.051 &   23.003 &   22.064 &   20.905 &    16.36 &     16.5 &    16.76 \\
      RSG 3335 &   308.8333385 &     60.1607698 &         308.83313 &           60.16085 &   27.584 &   24.959 &   99.999 &    21.28 &   20.177 &    17.23 &    17.35 &    14.59 \\
      RSG 3163 &   308.8340674 &     60.1686634 &         308.83399 &           60.16858 &   27.237 &   24.873 &   99.999 &   21.847 &   20.841 &    17.05 &    17.28 &    15.12 \\
      RSG 3336 &   308.8341101 &     60.1707295 &         308.83414 &           60.17065 &   27.633 &   24.882 &   22.864 &   21.171 &   20.188 &    17.21 &    17.35 &    16.67 \\
      RSG 3113 &   308.8403320 &     60.1721435 &         308.84054 &           60.17218 &   26.247 &   23.586 &   21.742 &   20.321 &   19.249 &    16.99 &    17.25 &    15.43 \\
\hline
\end{tabular}
\end{center}
\end{table}

%%%RIGHT HERE!!%%%

==> figset.tex <==
\figsetstart
% \figsetnum{18}
% \figsettitle{Remaining RGB Snapshots}

\figsetgrpstart
\figsetgrpnum{16.1}
\figsetgrptitle{RSG 767 - 9 Myr
}
\figsetplot{RSG_767.png}
\figsetgrpnote{Remaining 31 RGB Snapshots of 'A' labeled stars in the primary sample.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.2}
\figsetgrptitle{RSG 928 - 24 Myr
}
\figsetplot{RSG_928.png}
\figsetgrpnote{Remaining 31 RGB Snapshots of 'A' labeled stars in the primary sample.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.3}
\figsetgrptitle{RSG 1282 - 14 Myr
}
\figsetplot{RSG_1282.png}
\figsetgrpnote{Remaining 31 RGB Snapshots of 'A' labeled stars in the primary sample.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.4}
\figsetgrptitle{RSG 1321 - 15 Myr
}
\figsetplot{RSG_1321.png}
\figsetgrpnote{Remaining 31 RGB Snapshots of 'A' labeled stars in the primary sample.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.5}
\figsetgrptitle{RSG 1355 - 10 Myr
}
\figsetplot{RSG_1355.png}
\figsetgrpnote{Remaining 31 RGB Snapshots of 'A' labeled stars in the primary sample.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.6}
\figsetgrptitle{RSG 1534 - 4 Myr
}
\figsetplot{RSG_1534.png}
\figsetgrpnote{Remaining 31 RGB Snapshots of 'A' labeled stars in the primary sample.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.7}
\figsetgrptitle{RSG 1539 - 5 Myr
}
\figsetplot{RSG_1539.png}
\figsetgrpnote{Remaining 31 RGB Snapshots of 'A' labeled stars in the primary sample.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.8}
\figsetgrptitle{RSG 1661 - 5 Myr
}
\figsetplot{RSG_1661.png}
\figsetgrpnote{Remaining 31 RGB Snapshots of 'A' labeled stars in the primary sample.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.9}
\figsetgrptitle{RSG 1966 - 5 Myr
}
\figsetplot{RSG_1966.png}
\figsetgrpnote{Remaining 31 RGB Snapshots of 'A' labeled stars in the primary sample.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.10}
\figsetgrptitle{RSG 3335 - 13 Myr
}
\figsetplot{RSG_3335.png}
\figsetgrpnote{Remaining 31 RGB Snapshots of 'A' labeled stars in the primary sample.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.11}
\figsetgrptitle{RSG 4623 - 29 Myr
}
\figsetplot{RSG_4623.png}
\figsetgrpnote{Remaining 31 RGB Snapshots of 'A' labeled stars in the primary sample.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.12}
\figsetgrptitle{RSG 4881 - 27 Myr
}
\figsetplot{RSG_4881.png}
\figsetgrpnote{Remaining 31 RGB Snapshots of 'A' labeled stars in the primary sample.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.13}
\figsetgrptitle{RSG 2748 - 21 Myr
}
\figsetplot{RSG_2748.png}
\figsetgrpnote{Remaining 31 RGB Snapshots of 'A' labeled stars in the primary sample.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.14}
\figsetgrptitle{RSG 3335 - 13 Myr
}
\figsetplot{RSG_3335.png}
\figsetgrpnote{Remaining 31 RGB Snapshots of 'A' labeled stars in the primary sample.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.15}
\figsetgrptitle{RSG 3485 - 9 Myr
}
\figsetplot{RSG_3485.png}
\figsetgrpnote{Remaining 31 RGB Snapshots of 'A' labeled stars in the primary sample.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.16}
\figsetgrptitle{RSG 3532 - 29 Myr
}
\figsetplot{RSG_3532.png}
\figsetgrpnote{Remaining 31 RGB Snapshots of 'A' labeled stars in the primary sample.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.17}
\figsetgrptitle{RSG 5026 - 29 Myr
}
\figsetplot{RSG_5026.png}
\figsetgrpnote{Remaining 31 RGB Snapshots of 'A' labeled stars in the primary sample.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.18}
\figsetgrptitle{RSG 4906 - 11 Myr
}
\figsetplot{RSG_4906.png}
\figsetgrpnote{Remaining 31 RGB Snapshots of 'A' labeled stars in the primary sample.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.19}
\figsetgrptitle{RSG 2214 - 27 Myr
}
\figsetplot{RSG_2214.png}
\figsetgrpnote{Remaining 31 RGB Snapshots of 'A' labeled stars in the primary sample.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.20}
\figsetgrptitle{RSG 6822 - 12 Myr
}
\figsetplot{RSG_6822.png}
\figsetgrpnote{Remaining 31 RGB Snapshots of 'A' labeled stars in the primary sample.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.21}
\figsetgrptitle{RSG 3336 - 24 Myr
}
\figsetplot{RSG_3336.png}
\figsetgrpnote{Remaining 31 RGB Snapshots of 'A' labeled stars in the primary sample.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.22}
\figsetgrptitle{RSG 3091 - 7 Myr
}
\figsetplot{RSG_3091.png}
\figsetgrpnote{Remaining 31 RGB Snapshots of 'A' labeled stars in the primary sample.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.23}
\figsetgrptitle{RSG 4118 - 29 Myr
}
\figsetplot{RSG_4118.png}
\figsetgrpnote{Remaining 31 RGB Snapshots of 'A' labeled stars in the primary sample.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.24}
\figsetgrptitle{RSG 4480 - 27 Myr
}
\figsetplot{RSG_4480.png}
\figsetgrpnote{Remaining 31 RGB Snapshots of 'A' labeled stars in the primary sample.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.25}
\figsetgrptitle{RSG 4949 - 9 Myr
}
\figsetplot{RSG_4949.png}
\figsetgrpnote{Remaining 31 RGB Snapshots of 'A' labeled stars in the primary sample.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.26}
\figsetgrptitle{RSG 3954 - 11 Myr
}
\figsetplot{RSG_3954.png}
\figsetgrpnote{Remaining 31 RGB Snapshots of 'A' labeled stars in the primary sample.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.27}
\figsetgrptitle{RSG 2813 - 27 Myr
}
\figsetplot{RSG_2813.png}
\figsetgrpnote{Remaining 31 RGB Snapshots of 'A' labeled stars in the primary sample.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.28}
\figsetgrptitle{RSG 3561 - 17 Myr
}
\figsetplot{RSG_3561.png}
\figsetgrpnote{Remaining 31 RGB Snapshots of 'A' labeled stars in the primary sample.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.29}
\figsetgrptitle{RSG 6318 - 19 Myr
}
\figsetplot{RSG_6318.png}
\figsetgrpnote{Remaining 31 RGB Snapshots of 'A' labeled stars in the primary sample.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.30}
\figsetgrptitle{RSG 2171 - 17 Myr
}
\figsetplot{RSG_2171.png}
\figsetgrpnote{Remaining 31 RGB Snapshots of 'A' labeled stars in the primary sample.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.31}
\figsetgrptitle{RSG 2424 - 15 Myr
}
\figsetplot{RSG_2424.png}
\figsetgrpnote{Remaining 31 RGB Snapshots of 'A' labeled stars in the primary sample.}
\figsetgrpend

\figsetend
